The observable properties of galaxy accretion events in Milky Way-like galaxies in the FIRE-2 cosmological simulations

In the $\Lambda$-Cold Dark Matter model of the Universe, galaxies form in part through accreting satellite systems. Previous work have built an understanding of the signatures of these processes contained within galactic stellar halos. This work revisits that picture using seven Milky Way-like galaxies in the \textit{Latte} suite of FIRE-2 cosmological simulations. The resolution of these simulations allows a comparison of contributions from satellites above M$_{*}$$\gtrsim$10$\times$$^{7}$M$_{\odot}$, enabling the analysis of observable properties for disrupted satellites in a fully self-consistent and cosmological context. Our results show that, the time of accretion and the stellar mass of an accreted satellite are fundamental parameters that in partnership dictate the resulting spatial distribution, orbital energy, and [$\alpha$/Fe]-[Fe/H] compositions of the stellar debris of such mergers $at$ $present$ $day$. These parameters also govern the resulting dynamical state of an accreted galaxy at $z=0$, leading to the expectation that the inner regions of the stellar halo (R$_{\mathrm{GC}}$ $\lesssim$30 kpc) should contain fully phase-mixed debris from both lower and higher mass satellites. In addition, we find that a significant fraction of the lower mass satellites accreted at early times deposit debris in the outer halo (R$_{\mathrm{GC}}$ $>$50 kpc) that are $not$ fully phased-mixed, indicating that they could be identified in kinematic surveys. Our results suggest that, as future surveys become increasingly able to map the outer halo of our Galaxy, they may reveal the remnants of long-dead dwarf galaxies whose counterparts are too faint to be seen $in$ $situ$ in higher redshift surveys.

==> old_abstract.tex <==

In the $\Lambda$-Cold Dark Matter paradigm for the evolution of the Universe, galaxies form in part through accreting satellite systems. Analyses of prior simulations have built an understanding of the signatures of these processes contained within the stellar halos that surround galaxies. This work revisits that picture using a set of seven Milky Way(MW)-like galaxies in the \textit{Latte} suite of FIRE-2 zoom-in, baryonic, cosmological simulation. In particular, the resolution of these simulations allows a comparison of contributions from the most massive satellites with their lower mass counterparts (M$_{*}$$\gtrsim$10$\times$$^{7}$M$_{\odot}$); this enables the analysis of observable properties for disrupted satellites in a fully self-consistent and cosmological context. Our results confirm much of the physical insight developed in prior work focused on examining the mean properties of disrupted satellites. The time of accretion and the stellar mass of an accreted satellite system are fundamental parameters that in partnership dictate the resulting spatial distribution, orbital energy, and [$\alpha$/Fe]-[Fe/H] compositions of the stars belonging to the stellar debris of such mergers \textit{at present day}. These parameters also govern the resulting dynamical state of an accreted galaxy at $z=0$, leading to the expectation that the inner regions of the stellar halo (R$_{\mathrm{GC}}$ $\lesssim$30 kpc) should contain fully phase-mixed debris from both lower and higher mass satellites. In addition, we find that a significant fraction of the lower mass satellites accreted at early times deposit debris in the outer halo (R$_{\mathrm{GC}}$ $>$50 kpc). Moreover, these debris are {\it not} fully phased-mixed, indicating that they could be separated from the field halo population in kinematic surveys. Our results suggest that, as future surveys become increasingly able to map the outer halo of our Galaxy, they may reveal the remnants of long-dead dwarf galaxies whose counterparts are too faint to be seen {\it in situ} in higher redshift surveys. 
